LAMPRET: Layout-Aware Multimodal PreTraining for Document Understanding

Document layout comprises both structural and visual (eg. font-sizes) information that is vital but often ignored by machine learning models. The few existing models which do use layout information only consider textual contents, and overlook the existence of contents in other modalities such as images. Additionally, spatial interactions of presented contents in a layout were never really fully exploited. To bridge this gap, we parse a document into content blocks (eg. text, table, image) and propose a novel layout-aware multimodal hierarchical framework, LAMPreT, to model the blocks and the whole document. Our LAMPreT encodes each block with a multimodal transformer in the lower-level and aggregates the block-level representations and connections utilizing a specifically designed transformer at the higher-level. We design hierarchical pretraining objectives where the lower-level model is trained similarly to multimodal grounding models, and the higher-level model is trained with our proposed novel layout-aware objectives. We evaluate the proposed model on two layout-aware tasks -- text block filling and image suggestion and show the effectiveness of our proposed hierarchical architecture as well as pretraining techniques.

==> figs/block_sugg_viz.tex <==
\begin{figure}[ht!]
\centering
    \includegraphics[width=0.6\columnwidth]{figs/imgs/placeholder.png}
    \caption{
        \footnotesize
        \textbf{Block Suggestion Visualization:} caption.
    }
    \label{fig:block_sugg_viz}
\end{figure}

==> figs/img_sugg_viz.tex <==
\begin{figure}[ht!]
\centering
    \includegraphics[width=0.6\columnwidth]{figs/imgs/placeholder.png}
    \caption{
        \footnotesize
        \textbf{Image Suggestion Visualization:} caption.
    }
    \label{fig:img_sugg_viz}
\end{figure}

==> figs/teaser.tex <==
\begin{figure}[ht!]
\centering
    \includegraphics[width=0.6\columnwidth]{figs/imgs/placeholder.png}
    \caption{
        \footnotesize
        \textbf{Layout-Aware Document Representation Learning:} caption.
    }
    \label{fig:teaser}
\end{figure}

==> figs/templ.tex <==
\begin{figure}[ht!]
\centering
    \includegraphics[width=0.9\columnwidth]{figs/imgs/placeholder.png}
    \caption{
        \footnotesize
        \textbf{Fig:} caption.
    }
    \label{fig:fig}
\end{figure}

==> text/ethics.tex <==
% \clearpage

\raggedbottom

\section{Ethics and Broader Impacts}

We hereby acknowledge that all of the co-authors of this work are aware of the provided \textit{ACM Code of Ethics} and honor the code of conduct.
Particularly for this work, we believe our targeted impacts should lie in the communities of text mining, (multimodal) information retrieval, document understanding and compositions. The followings are addressing specifically for our NLP applications:

\vspace{0.3em}

\mypar{Intended Use:} The intended use of our work is broadly (multimodal) document understanding and spurring research in novel document compositions anchoring around an intended structural layout. The community specifically in document processing and/or retrieval should benefit from our work. We urge the users to be careful if training on documents with hateful speech or non-ethical images, and kept the resulting composed documents, if any, private, to prevent from harming any groups and societies.

\vspace{0.3em}

\mypar{Failure Mode:} We do not anticipate specific failure modes in our work, and the potential harms can, and should be, sufficiently taken care of by carefully using of the training data.

\vspace{0.3em}

\mypar{Biases:} Currently our pretrained models are trained on Wikipedia, and we do not specifically only collect Wikipages from a limited set of genres. As a result, we believe our models are not specifically biased towards any topics, unless trained on different sets of documents with very limited diversity. Again such an issue can be alleviated by carefully designing what data to train on.

\vspace{0.3em}

\mypar{Misuse potential:} If the above intended use and biases are properly and carefully taken care of, we anticipate our models would not be misused with unethical intentions.

\vspace{0.3em}

\mypar{Collecting data from users:} Since our system can learn from any kinds of written online documents, we restate that the models should be handled with cautious if trained on potentially harmful speech. We hope our work inspires the research on better document understanding and compositions, for creating novel but ethical documents.

\vspace{0.3em}

\mypar{Potential harm to vulnerable populations:} Unless specifically targeting those populations with unethical intentions, we do not anticipate our work would harm any vulnerable populations.
